Towards Closing the Energy Gap Between HOG and CNN Features for Embedded Vision

Computer vision enables a wide range of applications in robotics/drones, self-driving cars, smart Internet of Things, and portable/wearable electronics. For many of these applications, local embedded processing is preferred due to privacy and/or latency concerns. Accordingly, energy-efficient embedded vision hardware delivering real-time and robust performance is crucial. While deep learning is gaining popularity in several computer vision algorithms, a significant energy consumption difference exists compared to traditional hand-crafted approaches. In this paper, we provide an in-depth analysis of the computation, energy and accuracy trade-offs between learned features such as deep Convolutional Neural Networks (CNN) and hand-crafted features such as Histogram of Oriented Gradients (HOG). This analysis is supported by measurements from two chips that implement these algorithms. Our goal is to understand the source of the energy discrepancy between the two approaches and to provide insight about the potential areas where CNNs can be improved and eventually approach the energy-efficiency of HOG while maintaining its outstanding performance accuracy.

==> 4_performance_comparison.tex <==
%% ====================================================================
\section{Performance Comparison}
\label{sec:performance_comparison}
%% ====================================================================

In this section, complete object detection systems are analyzed with object detection accuracy numbers. As shown below, different classification techniques lead to different accuracy numbers. The mean Average Precision (mAP) metric is used to measure the accuracy.

%% ====================================================================
%\subsection{Different Object Detection Approaches}
%\label{sec:different_detection_approaches}
%% ====================================================================
%For HOG hand-crafted features, a simple detection approach is to train an SVM classifier that captures the characteristics of the object of interest, and sweep the entire images at all position to locate the object. This is the method used in the original HOG paper~\cite{dalal2005histograms}. To increase the detection accuracy, a more complex approach is used in~\cite{girshick2012discriminatively}, called deformable parts models (DPM), where few extra SVM classifier are trained to detect moving parts and allow object deformation. With its flexibility, the DPM object detection achieves 2$\times$ higher detection accuracy compared to rigid body models. However, this comes at a 35$\times$ computation overhead~\cite{suleiman201658}.

%With learned CNN features, some examples of object detection with CNN features are presented in~\cite{zou2014dnp, girshick2015dpmcnn, cvpr2014-girshick, girshick2015frcnn}. In these approaches, the output of the convolution layers is used as input features to the classifiers. Different classification approaches are used with CNN features. For instance, boosting classifier cascades are used in~\cite{zou2014dnp}, while a separate convolution layer is used in~\cite{girshick2015dpmcnn} as a classifier. The most common classification approach with CNN is using fully connected layers with Softmax as done in~\cite{cvpr2014-girshick, girshick2015frcnn}.

%% ====================================================================
\subsection{Complexity}
\label{sec:complexity}
%% ====================================================================
Tables~\ref{tab:feat_comp} and~\ref{tab:feat_energy} show the computation requirements and the measured energy consumption to extract the two types of features. For learned features, two CNN architectures (i.e., AlexNet and VGG) are implemented on Eyeriss chip to show its flexibilty to adapt to different CNN architectures. Comparing between hand-crafted and learned features, Table~\ref{tab:feat_comp} shows a one to two orders of magnitude computation difference. This difference is justified with the higher dimensionality of the learned features. However, a much larger two to four orders of magnitude energy consumption difference is shown in Table~\ref{tab:feat_energy}. The two types of programmability, i.e., PoP and PoHP, discussed in Section~\ref{sec:hardware_considerations} are believed to be the main reason for the gap between computation and energy. The HOG features extraction architecture is hardwired with no PoP and PoHP in order to achieve the highest possible energy efficiency. In contrast, the CNN accelerator has both PoP and PoHP, so it can be programmed to implement different CNN architectures with user-defined parameters.

\begin{table}
    \begin{center}
        \normalsize
        \caption{Features computation.}
        \begin{tabular}{|l|c|c|c|} \hline
            \multicolumn{2}{|c|}{\textbf{Feature}}&\textbf{GOP/Mpixel}&\textbf{Ratio}\\ \hline
            \multicolumn{2}{|c|}{Hand-crafted HOG~\cite{suleiman201658}}&0.7&1.0$\times$\\ \hline
            \multirow{2}{*}{Learned~\cite{isscc2016-chen}}&AlexNet&25.8&36.9$\times$\\ \cline{2-4}
            &VGG&610.3&871.9$\times$\\ \hline
        \end{tabular}
        \label{tab:feat_comp}
    \end{center}
    %\vspace{-5pt}
\end{table}

\begin{table}
    \begin{center}
        \normalsize
        \caption{Features extraction energy consumption.}
        \begin{tabular}{|l|c|c|c|} \hline
            \multicolumn{2}{|c|}{\textbf{Feature}}&\textbf{Energy {\small (nJ/pixel)}}&\textbf{Ratio}\\ \hline
            \multicolumn{2}{|c|}{Hand-crafted HOG~\cite{suleiman201658}}&0.5&1.0$\times$\\ \hline
            \multirow{2}{*}{Learned~\cite{isscc2016-chen}}&AlexNet&155.5&311.0$\times$\\ \cline{2-4}
            &VGG&6,742.9&13,485.8$\times$\\ \hline
        \end{tabular}
        \label{tab:feat_energy}
    \end{center}
    %\vspace{-5pt}
\end{table}

%% ====================================================================
\subsection{Detection Accuracy vs. Energy Efficiency}
\label{sec:accuracy_vs_energy}
%% ====================================================================
Fig.~\ref{fig:hand_vs_dnn} shows the trade-off between detection accuracy and energy consumption. Note that the vertical axis is in logarithmic scale. All reported detection accuracy numbers are measured on PASCAL VOC 2007 dataset~\cite{pascal-voc-2007}, which is a widely used image dataset containing 20 different object classes in 9,963 images. The same accuracy of HOG based object detection can be achieved using the output of the third convolution layer of AlexNet with the object detection pipeline in~\cite{zou2014dnp}, but a 100$\times$ more energy is required to generate the learned features. Fortunately, mAP can be doubled by using the output of the fifth and final convolution layer of AlexNet, with minimal increase in the energy consumption (only 22\%). For much higher mAP, authors in~\cite{girshick2015frcnn} use VGG CNN which has more convolution layers compared to AlexNet. However, the energy consumption of VGG is four orders of magnitudes higher than HOG features. Fig.~\ref{fig:hand_vs_dnn} shows that for a linear increase in the detection accuracy, an exponential increase in energy consumption is required.


\begin{figure}
    \begin{center}
        \includegraphics[width=0.9\linewidth]{figures/hand_vs_dnn_new.pdf}
        \caption{    Energy versus accuracy trade-off comparison for hand-crafted and learned features.
                }
        \vspace{-10pt}                
        \label{fig:hand_vs_dnn}
    \end{center}
\end{figure}

